Higher-order models for glioma invasion: from a two-scale description to effective equations for mass density and momentum

Starting from a two-scale description involving receptor binding dynamics and a kinetic transport equation for the evolution of the cell density function under velocity reorientations, we deduce macroscopic models for glioma invasion featuring partial differential equations for the mass density and momentum of a population of glioma cells migrating through the anisotropic brain tissue. The proposed first and higher order moment closure methods enable numerical simulations of the kinetic equation. Their performance is then compared to that of the diffusion limit. The approach allows for DTI-based, patient-specific predictions of the tumor extent and its dynamic behavior.

==> Sections/modelling.tex <==
\section{General models}
\label{section1a}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We consider a slightly generalized version of equation (\ref{KTE}).
Let $$x \in \R^3, v  \in V=S^2, z \in Z \subset \R.$$
The distribution function is $f=f(x,v,z,t)$, the  density
$$\rho= \rho(x,z,t) = \int_V f(x,v,z,t) d v .$$
We consider
\begin{align}
\label{pdegeneral}
\partial_t f  + v \cdot \nabla_x f + \partial_z (G f ) &= L f -\lambda_A f
\end{align}
with
the definitions 
$$L = L_1 + L_2 $$ and for $i=1,2$ 
\begin{align}
L_i f =  \int_V \left( k_i(v,v^\prime) f(v^\prime) -  k_i( v^\prime,v) f (v) \right) d v^\prime.
\end{align}
Here, 
$\lambda_A = \lambda_A(z)$, $G = G(x,v,z)$ and $L_i f = L_i f (x,v,z,t)$ and $k_i = k_i (v,v^\prime) = k_i (v,v^\prime,z) $.
We assume 
% % \int_V v^\prime k_1(v^\prime,v)  dv^\prime =0
%$$
$$
\int_V  k_1(v^\prime,v)  dv^\prime = \lambda= \lambda(z).
$$
Moreover,we assume that there is an equilibrium distribution  $F= F (x,v)$,  fulfilling the detailed balance condition
\begin{align}
k_1(v^\prime,v)F (v) = k_1(v, v^\prime)F (v^\prime)
\end{align}
and
\begin{align}
\int_V F (v) dv =1.
\end{align}
We note that this yields
$$
tr [\int_{S^2} v \otimes v F(v) dv  ] =1
$$


%\begin{remark}
%Moreover, we consider $G$ such that $Y$ is an invariant set of the evolution of $\dot{y} = G(y)$.
%\begin{align}
%G(y) = (a (R_0 - y_1 - y_2 ) - b y_1, c (R_0 -y_1-y_2) -  d y_2)
%\end{align}
%with constants $a,b,c,d$.
%\end{remark}




Examples for the collision kernels $k$ are  given by
	\begin{align}
	k(v, v^\prime) = \lambda F(v) .
	\end{align}
	In particular,  a model for a haptotaxis kernel is given by 
	$F(v) = \hat Q(v) $. This  yields
	\begin{align}
	Lf(v) = -  \lambda  \left(f-   \rho \hat Q(v) \right) .
	\end{align}
	More general  haptotaxis type kernels are given by
	\begin{align}
	k(v, v^\prime) =  \lambda_H\int_{V} \psi(v,v^\prime,\theta^\prime) \hat{Q} (\theta^\prime) d  \theta^\prime.
	\end{align}

	
	A further example is given by a chemotaxis type kernel
	\begin{align}
	k(v, v^\prime) = ( a v - b v^\prime ) F(v)
	\varphi(\nabla m )
	\end{align}
	with constants $a $ and $b$.
	We obtain
	\begin{align}
	L f (v) = \left( a (\rho v F(v) - \int  v F dv   f)+ b (vf - \rho u F(v)) \right)  \varphi(\nabla m ).
	\end{align}
	The flux-limiter $\varphi$ is chosen for example as 
	\begin{align}
	\varphi(x) =  \frac{x}{\sqrt{1+\vert x \vert^2 }}
	\end{align}
	or
	$\varphi (x) =(\frac{\vert x \vert - s^\star}{\sqrt{1+ (\vert x \vert- s^\star)^2}} +s^\star) \frac{x}{\vert x \vert}$,
	compare \cite{}. 
	
The  equation for the chemoattractant  
	%for the fibre distribution $Q = Q(t,x,v)$ 
	%\begin{align}
	%\partial_t Q (v) = \gamma m \left(  \int_V \vert v \cdot v^\prime \vert
	%\int_Y f(v^\prime,y) dy  dv^\prime  - \bar{\rho} \right)  Q(v)  
	%\end{align}
  $m = m(t,x)$ is given by 
	\begin{align}
	\partial_t m - D_m \Delta_x m = \eta \hat Q \int \rho dz    - \delta m  .
	\end{align}
	



\begin{remark}{Example (Glioma).}
	
	We consider the reduced kinetic equation derived in the previous section.
	With $\lambda_A =0$ and $G=0$ in (\ref{pdegeneral}) and 
	$$
	k_1 = \lambda_H \hat Q(v)
	$$ and $$k_2=-  \tilde \lambda_H \cdot v^\prime \hat Q(v)$$  we obtain equation (\ref{glioma}).
%	\begin{align}
%	\partial_t f  + v \cdot \nabla_x f  = - \lambda_H \left( f- \hat Q  \right)  + \tilde \lambda_H \cdot (v f -  \hat Q(v)q ) 
%	\end{align}
	
%	\begin{align}
%	\partial_t f  + v \cdot \nabla_x f  = - \lambda_H \left( f- \hat Q  \right)  + \tilde \lambda_H \cdot (v f -  \hat Q(v)q ) \\
%	\partial_t m - D_m \Delta_x m = \eta {\rho} <Q>    - \delta m \\
%	\partial_t Q   = \gamma m \left(  \int_V \vert v  \cdot v^\prime \vert
%	f(v^\prime)   dv^\prime  - \rho \right)  Q   
%	\end{align}
%	
\end{remark}



\section{Diffusion limit}

We derive an equation for $$\rho = \int_V f(v) d v $$ under the assumption
	\begin{align}
		\int_V v F (v) dv =0.
	\end{align}
For $F(v) = \hat Q(v)$  this means that the fibers have no preferred direction, that means  the fibre distribution $\hat Q$ is first order symmetric.

Start with a scaled version of the kinetic equation
\begin{align}
\label{pdeinitialscaled}
\epsilon^2 \partial_t f  + \epsilon v \cdot \nabla_x f + \epsilon^2 \partial_z  (G f ) &= (L_1  
+ \epsilon L_2 ) f  -  \epsilon^2 \lambda_A f
\end{align}
and use
$$
f = f_0 + \epsilon f_1 + \cdots .
$$
Then to zeroth order
\begin{align}
L_1 f_0 = 0 
\end{align}
with the solution
$$
f_0 (v)= \rho_0  F (v)
$$
To first order
\begin{align}
\label{firstorder}
v \cdot \nabla_x f_0 = L_1 f_1
+  L_2 f_0
\end{align}
or
\begin{align}
L_1 f_1=     v  \cdot \nabla_x (F(v)\rho_0) 
-\rho_0 L_2 F 
\end{align}
Since
$$
\int_V v F(v) d v =0, \int_V v \nabla_x F(v) d v =0, \int_V L_2 F (v) d v =0
$$
this is solvable.
Then
\begin{align}
f_1 =   -   H_1(v) \cdot \nabla_x \rho_0 (y) 
+ \rho_0 H_2(v) 
\end{align}
where
\begin{align}
L_1 H_1 (v)=  -  v F(v)\\
L_1 H_2(v)=  -  L_2 F (v) - v \nabla_x F(v).
\end{align}

Integrate with respect to $v$:
\begin{align}
\partial_t \rho_0  +   \nabla_x \cdot \int_V  v f_1 dv + \partial_z (G_F \rho_0 ) &= -\lambda_A \rho_0
\end{align}
or
\begin{align}
\partial_t \rho_0  -    \nabla_x \cdot \left( D \nabla_x     \rho_0  -   \Gamma   \rho_0  \right) 
+ \partial_z (G_F \rho_0 ) 
=-\lambda_A
\rho_0
\end{align}
with
\begin{align}
D =   \int_V  v \otimes  H_1(v)  dv \\
\Gamma = \int_V  v H_2(v)  dv
\end{align}
and
$$
G_F = \int_V G(v,y) F(v) dy
$$

%Using in the $Q$-equation
%$f = f_0 = \rho_0  F (v)$ we get
%\begin{align}
%\partial_t Q(v)  = \gamma m \left(  \int_V \vert v \cdot v^\prime \vert
%\int_Y \rho_0 (y) dy F(v^\prime)  dv^\prime  -  \bar{\rho_0} \right)  Q(v)   
%\end{align}
%We write 
%\begin{align*}
%\partial_t Q  = \gamma   S_F
%\bar \rho_0 m Q
%\end{align*}
%with  $$S_F = S_F(v) = \int_V \left(\vert v \cdot v^\prime \vert-1  \right) F(v^\prime) dv^\prime$$
%The last equation can be solved explicitely, we obtain 
%\begin{align}
%Q (v,t) = Q(v,0) \exp{\left(\gamma S_F(v) \int_0^t \bar \rho_0(t^\prime) m(t^\prime) d t^\prime \right)}.
%\end{align}


\begin{remark}
	Scaling the Glioma  equation (\ref{glioma}) gives 
	
	\begin{align}
	\label{gliomascaled}
	\epsilon^2 \partial_t f  + \epsilon v \cdot \nabla_x f 
	= - \lambda_H \left(f - \hat Q(\hat v) \rho \right) +  \epsilon \tilde \lambda_H  \left(v  q - \hat Q (\hat v) q  \right).
	\end{align}
	We obtain 
	\begin{align}
	\lambda_H  \left( H_1 - \int_V H_1 dv  \hat Q(v) \right)  =    v  \hat Q(v)   
	\end{align}
	and therefore
	\begin{align}
	H_1   =   - \frac{1}{ \lambda_H}  v  \hat Q(v) 
	\end{align}
	Moreover,
	\begin{align}
	L_2 F (v)  =  \tilde \lambda_H \cdot v   \hat Q(v) 
	\end{align}
	and
	\begin{align}
	H_2  = 
	\frac{\tilde \lambda_H}{\lambda_H} \cdot v \hat Q(v)
	+  \frac{1}{\lambda_H}  v \cdot \nabla_x \hat Q(v)
	\end{align}
	
	This gives 
	\begin{align}
	D  &= \frac{1}{ \lambda_H } \int_V  v \otimes v \hat Q(v)  dv 
	= \frac{1}{ \lambda_H } D_{\hat Q}
	\\
	\Gamma  & = \frac{1}{ \lambda_H } \int_V  v \otimes v \hat Q(v)  dv \tilde \lambda_H +
	\frac{1}{ \lambda_H}  \nabla_x \cdot \int_V  v \otimes v \hat Q(v)  dv
	= D  \tilde \lambda_H + \nabla_x \cdot D
	\end{align}
	and finally
	\begin{align*}
	\partial_t \rho  -   \nabla_x \cdot \left( \nabla_x \cdot (\rho D)  
	-   \rho D \tilde \lambda_H  \right)
	=0
	\end{align*}
We refer again to \cite{}.	
%	together with 
%	\begin{align*}
%	\partial_t Q  = \gamma   S_Q
%	\bar \rho_0 m Q
%	\end{align*}
\end{remark}

==> symbols.tex <==
%----------------------------------------------------------------------------------------
%   COMMON SYMBOLS
%----------------------------------------------------------------------------------------

\newcommand{\xmip}[2]{x^{#1}_{#2}}
%\newcommand{\bn}{{\bf n}}
%\newcommand{\be}{\begin{eMnarray}}
	%\newcommand{\ee}{\end{eMnarray}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\om}{\omega }
\newcommand{\tr}{\mbox{tr}}
\newcommand{\quand}{\mbox{and}}
